Coordination in Categorical Compositional Distributional Semantics

An open problem with categorical compositional distributional semantics is the representation of words that are considered semantically vacuous from a distributional perspective, such as determiners, prepositions, relative pronouns or coordinators. This paper deals with the topic of coordination between identical syntactic types, which accounts for the majority of coordination cases in language. By exploiting the compact closed structure of the underlying category and Frobenius operators canonically induced over the fixed basis of finite-dimensional vector spaces, we provide a morphism as representation of a coordinator tensor, and we show how it lifts from atomic types to compound types. Linguistic intuitions are provided, and the importance of the Frobenius operators as an addition to the compact closed setting with regard to language is discussed.

==> eptcsdata.tex <==
\providecommand{\firstpage}{29}
\providecommand{\publicationstatus}{Kartsaklis, D., Lewis, M. and Rimell, L. (Eds):\\2016 Workshop on Semantic Spaces at the Intersection of\\NLP, Physics and Cognitive Science (SLPCS'16)\\
EPTCS 221, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.221.4}{10.4204/EPTCS.221.4}}

